Faster and better: a machine learning approach to corner detection

The repeatability and efficiency of a corner detector determines how likely it is to be useful in a real-world application. The repeatability is importand because the same scene viewed from different positions should yield features which correspond to the same real-world 3D locations [Schmid et al 2000]. The efficiency is important because this determines whether the detector combined with further processing can operate at frame rate. Three advances are described in this paper. First, we present a new heuristic for feature detection, and using machine learning we derive a feature detector from this which can fully process live PAL video using less than 5% of the available processing time. By comparison, most other detectors cannot even operate at frame rate (Harris detector 115%, SIFT 195%). Second, we generalize the detector, allowing it to be optimized for repeatability, with little loss of efficiency. Third, we carry out a rigorous comparison of corner detectors based on the above repeatability criterion applied to 3D scenes. We show that despite being principally constructed for speed, on these stringent tests, our heuristic detector significantly outperforms existing feature detectors. Finally, the comparison demonstrates that using machine learning produces significant improvements in repeatability, yielding a detector that is both very fast and very high quality.

==> thesis_introduction.tex <==
\def\CornerResponse{\ensuremath{C}\xspace}
\def\Image{\ensuremath{I}\xspace}


\section{Introduction}

\PARstart{C}{orner} detection is used as the first step of many vision tasks such as
tracking, localisation, SLAM (simultaneous localisation and mapping), image
matching and recognition.  This need has driven the development of a large
number of corner detectors.  However, despite the massive  increase in
computing power since the inception of corner detectors, it is still true that
when processing live video streams at full frame rate, existing feature
detectors leave little if any time for further processing.

In the applications described above, corners are typically detected and matched
into a database, thus it is important that the same real-world points are
detected repeatably from multiple views \cite{schmid2000comparing}. The amount
of variation in viewpoint under which this condition should hold depends on the
application.  

\section{Previous work}

\subsection{Corner detectors}

Here we review the literature to place our advances in
context.  
The term ``corner'' refers to a small
point of interest with variation in two dimensions.
Such points often arise as the result of geometric
discontinuities, such as the corners of real world objects, but they may also
arise from small patches of texture. Most algorithms are capable of detecting
both kinds of points of interest, though the algorithms are often  designed to
detect one type or the other.
A number of the detectors described below compute a corner response,
\CornerResponse, and define corners to be large local maxima of \CornerResponse.


\subsubsection{Edge based corner detectors}

An edge (usually a step change in intensity) in an image corresponds to the
boundary between two regions.  At corners, this boundary changes
direction rapidly. Many techniques were developed which involved detecting and
chaining edges to extract curves and defining corners as high curvature points.
Such curves are highly
quantized, so early methods used a chord of the curve to compute the slope and
defined curvature as rate of change of slope~\cite{rosenfeld73angle}. More
recently, Gaussian smoothing has been used to avoid problems with quantization.
The Curvature Scale Space~\cite{CSS} smooths contours with a scale proportional
to the length.  The radius of curvature of the contour is computed and corners
are detected as maxima of curvature where the maxima are significantly larger
than the closest minima.  Instead of direct smoothing, edges can be
parameterised with cubic splines and corners detected at rapid 
changes in the first derivative where there is a large deviation of the  spline 
from the control point~\cite{langridge-corner,medioni-corner}.

One of the problems with chained edge techniques is the reliance on the method
used to perform segmentation and chaining of the contours.  Instead of this
approach, many other techniques look for rapid changes on an edge by detecting
edge points (edgels) and then examining the local edge or image properties
instead.  By finding both edges and their directions, a patch on an edge can be
compared to patches on either side in the direction of the contour, to find
points with low self-similarity~\cite{cooper-corner}.

Rapid changes in
the edge direction can be found by measuring the derivative of the gradient direction along
an edge, multiplied by the magnitude of the gradient, giving a score of:
\begin{align}
\label{eqn:kitchen}
\CornerResponse_K&=\frac{g_{xx}g_y^2 + g_{yy}g_x^2 - 2g_{xy}g_xg_y}{g_x^2g_y^2}\\
\intertext{where, in general,}
g_x &= \pdif{g}{x},\quad g_{xx} = \pdif[2]{g}{x^2}, \quad \text{etc\dots}\notag,
\end{align}
and $g$ is either the image or a bivariate polynomial (optimally quadratic)
fitted locally to the image~\cite{kitchen-rosenfeld-corner}.
If edgels are only detected at the steepest part of an edge, then a
score computing total image curvature at the edgels is given by:
\begin{equation}
	\CornerResponse_W = \grad^2\Image - S\abs{\grad\Image}^2.
	\label{eqn:wang}
\end{equation}
where $\grad\Image$ is the image gradient~\cite{wang-brady-corner} and $S$ is a
parameter.


\subsubsection{Greylevel derivative based detectors}

The assumption that corners exist
along edges is an inadequate model for patches of texture and point like
features, and is difficult to use at `T'-junctions.  Therefore a large number of
detectors operate directly on greylevel images without requiring edge
detection.

Beaudet~\cite{beaudet78corner} defines corners to be local extrema in the determinant
of the Hessian:
\begin{equation}
	C_\text{DET} = |\hessian{I}| = I_{xx}I_{yy} - (I_{xy})^2.
\end{equation}
This is frequently referred to as the DET operator. 


Features can be defined as points with low self-similarity in all directions.
The self-similarity of an image patch can be measured by taking the SSD (sum of
squared differences) between an image patch and a shifted version of
itself~\cite{moravec_1980}.  The image patch is shifted horizontally,
vertically and along the two diagonals and $C$ is defined to be the smallest
SSD. This is the basis for a large class of detectors.  Harris and
Stephens~\cite{Harris88Corner} built on this by computing an approximation to
the second derivative of the SSD with respect to the shift.  This is both
computationally more efficient and can be made isotropic. The result is:
\def\Harris{\Mat{H}}
\begin{equation}
{
\label{eqn:harrismatrix}
\def\id#1{\pdif{I}{#1}}
\Harris = \left[
\begin{array}{cc}
\widehat{I_x^2} & \widehat{I_xI_y}\\
\widehat{I_xI_y} & \widehat{I_y^2} 
\end{array}
\right],
}
\end{equation}
where $\ \widehat{}\ $ denotes averaging performed over the area of the image
patch. Further, Harris uses a smooth circular window over which to perform the
averaging which results in an isotropic and less noisy response.

Because of the wording used in \cite{Harris88Corner}, it is often mistakenly
claimed that \Mat{H} is equal to the negative second derivative of the
autocorrelation. This is not the case because the SSD is equal to the sum of the
autocorrelation and some additional terms~\cite{rosten_2006_thesis}.


Harris defines the corner response to be:
\begin{equation}
\label{eqn:harris}
\CornerResponse_H = |\Harris| - k (\operatorname{trace}
\Harris)^2. 
\end{equation}
This is large if both eigenvalues are large, and it avoids explicit
computation of the eigenvalues. It has been shown~\cite{noble-corners} that this
is an approximate measure of the image curvature, though the approximation is
different to the one used in (\ref{eqn:kitchen}) and (\ref{eqn:wang}).

The earlier F\"{o}rstner~\cite{forstner86feature} algorithm is easily explained in
terms of \Harris:
\begin{equation}
\CornerResponse_F = \left\{
						\begin{array}{ll}
							\frac{|\Harris|}{\operatorname{trace}\Harris}, & \text{if}\ \frac{|\Harris|}{(\operatorname{trace}\Harris)^2} > t \\
							0  & \text{otherwise}
						\end{array}
					\right.,
\end{equation}
where $t$ is a threshold.

Under affine motion, it is better to use
the smallest eigenvalue of \Harris as the corner strength
function~\cite{shi93good}:
\begin{equation}
\CornerResponse_S=\operatorname{min}\ \lambda_1,\lambda_2.
\end{equation}
A number of other suggestions
\cite{Harris88Corner,noble-descriptions,shi93good,Kenney03-condition} have been
made for how to compute the corner strength from \Harris, and these have been
shown to all be equivalent to various matrix norms of
\Harris~\cite{Zuliani04-MathematicalComparison}.
The number of channels and  image dimensionality can be generalized
~\cite{kenney05axiomatic}, and it can be shown that
\cite{forstner86feature,shi93good,rohr97differential} are equivalent to specific
choices of the measure used in \cite{Kenney03-condition}.


\Harris can also be generalized by considering a template matching scheme with
a pointwise comparison which behaves similarly to the SSD (sum of squared
differences) for small differences. The stability with respect to the match
parameters can be computed,  and the result is a generalization of \Harris
(where \Harris is maximally stable for no appearance model, linear translation
and SSD matching). This is used to derive detectors which will give points
maximally stable for template matching, given similarity transforms,
illumination models and prefiltering~\cite{triggs04keypoints}.

An alternative approach to the problem of finding a scalar value which measures
the amount of second derivative is to take the Laplacian of the image. To
reduce the amount of noise (second derivatives greatly amplify noise), the
smoothed Laplacian is computed by convolving the image with the LoG (Laplacian
of a Gaussian).  Since the LoG kernel is symmetric, an alternative
interpretation is that this is performing matched filtering for features which
are the same shape as a LoG. As a result, the variance of the Gaussian
determines the size (or scale) of features of interest.  It has been
noted~\cite{affine-schmid} that the locations of maxima of the LoG over
different scales are particularly stable.

Scale invariant corners can be extracted by convolving the image with a DoG
(Difference of Gaussians) kernel at a variety of scales (three per octave) and
selecting local maxima in space and scale~\cite{SIFT}.  DoG is a good
approximation for LoG and is much faster to compute, especially as the
intermediate results are useful for further processing.  To reject edge-like
features, the eigenvalues of the Hessian of the image are computed and features
are kept if the eigenvalues are sufficiently similar (within a factor of 10).
This method can be contrasted with \Eqn{wang}, where the Laplacian is compared
to the magnitude of the edge response.  If two scales per octave are
satisfactory, then a significant speed increase can be achieved by using
recursive filters to approximate Gaussian convolution~\cite{crowley03fast}.

Harris-Laplace~\cite{harris-laplace} features are detected using a similar
approach. An image pyramid is built 
and features are detected by computing
$\CornerResponse_H$  at each layer of the pyramid.  Features are
selected if they are a local maximum of  $\CornerResponse_H$ in the image plane
and a local maxima of the LoG across scales.

Recently, scale invariance has been extended to consider features which are
invariant to affine transformations
\cite{affine-schmid,lowe-brown-affine,affine_features,zisserman-affine}.
However, unlike the 3D scale space, the 6D affine space is too large to search,
so all of these detectors start from corners detected in scale space. These in
turn rely on 2D features selected in the layers of an image pyramid.

\subsubsection{Direct greylevel detectors}

Another major class of corner detectors work by examining a small patch of an
image to see if it ``looks'' like a corner. The detector presented in this paper
belongs to to this class of detectors.  Since derivatives are not computed, a
noise reduction step, such as Gaussian smoothing, is not required.  The result
of this is that some of these corner detectors are computationally efficient
since they only examine a small number of pixels for each corner detected. A
corollary of this is that they tend to perform poorly on images with only large
scale features (such as blurred images).  The detectors described below are the
most closely related to the techniques described in this paper. 


A number of techniques assume
that a corner has the general appearance of one or more wedges of a uniform
intensity. Using this model, a response function can be derived using local
Zernike moments~\cite{ghosal94corner}.  Alternatively, if a corner is a wedge,
then it will have concentric contiguous arcs of pixels which are significantly
different from the centre pixel~\cite{shen00real}. 

The tip of a wedge is not self-similar, so this can be generalized by defining
corners as points which are not self-similar.  The proportion of pixels in a
disc around a centre (or \term{nucleus}) which are similar to the centre is a
measure of self similarity. This is the USAN (univalue segment assimilating
nucleus).  Corners are defined as SUSAN (smallest USAN, \ie local minima) points
which also pass a set of rules to suppress qualitatively bad features. In
practice, a weighted sum of the number of pixels inside a disc whose intensity
is within some threshold of the centre value is used~\cite{Smith97SUSAN}.

Self similarity can be measured using  a circle instead of a
disc~\cite{Trajkovic-Headley-fast}. The SSD between the center pixel and the
pixels at either end of a diameter line is an oriented measure of
self-dissimilarity. If this is small in any orientation then the point is not a
corner. This is computationally efficient since the process can be stopped as
soon as one small value is encountered.

All the detectors described above define corners using a model or algorithm and
apply that algorithm directly to the image.  An alternative is to train a
classifier on the model and then apply the classifier to the image.  For
instance, in \cite{dias95neural1}, a three layer neural network is trained to
recognise corners where edges meet at a multiple of 45\degree, near to the
centre of an $8\times8$ window. This is applied to images after edge detection
and thinning.  


%If a classifier is used, then it does not have to be trained directly on a
%specific model. The classifier can be trained on
%Instead of using a model, Kienzle
%\etal~\cite{kienzle05interest} use human perception.  Images are shown to a
%number of test subjects. Image locations which are consistently fixated on (as
%measured by an eye tracking system) are taken to be interesting, and a support
%vector machine is trained to recognize these points.

If a classifier is used, then it can be trained according to how a corner should
behave, \ie that its performance in a system for evaluating detectors should be
maximized.  Trujillo and Olague \cite{trujillo06synthesis} state that detected
points should have a high repeatability (as defined by
\cite{schmid2000comparing}), be scattered uniformly across the image and that
there should be at least as many points detected as requested.  A corner
detector function is optimized (using genetic programming) to maximize the score
based on these measures.


The FAST-$n$ detector (described in \Sec{st}) is related to the
wedge-model style of detector evaluated using a circle surrounding the candidate
pixel.  To optimize the detector for speed, this model is used to train a
decision tree classifier and the classifier is applied to the image.  The
FAST-ER detector (described in \Sec{FASTER}) is a generalization which allows
the detector to be optimized for repeatability.



\subsection{Comparison of feature detectors}


Considerably less work has been done on comparison and evaluation of feature
detectors than on inventing new detectors.  The tests fall into three broad
categories (tests for the localisation accuracy are not considered here since
for most applications the presence or absence of useful corners is the limiting
factor): \begin{enumerate}

\item {\em Corner detection as object recognition.} Since there is no good
definition of exactly what a corner should look like, algorithms can be compared
using simplistic test images where the performance is evaluated (in terms of
true positives, false positives, etc\ldots) as the image is altered using
contrast reduction, warps and added noise.  Since a synthetic image is used,
corners exist only at known locations, so the existence of false negatives and
false positives is well defined. However, the method and results do not
generalize to natural images. 

\item {\em System performance.}
The performance of an application (often tracking) is evaluated as the corner
detector is changed. The advantage is that it tests the suitability of detected
corners for further processing.  However, poor results would be obtained from a
detector ill matched to the downstream processing. Furthermore the results do
not necessarily generalize well to other systems. To counter this, sometimes
part of a system is used, thouth in this case the results do not necessarily
apply to any system.

\item {\em Repeatability.} This tests whether corners are detected from multiple
views. It is a low level measure of corner detector quality and provides an
upper bound on performance. Since it is independent of downstream processing,
the results are widely applicable, but it is possible that the detected features
may not be useful. Care must be used in this technique, since the trivial
detector which identifies every pixel as a corner achieves 100\% repeatability.
Furthermore, the repeatability gives no indication as
to the usefulness of the detected points for further processing. For instance,
the brightest pixels in the image are likely to be repeatable but not especially
useful.
\end{enumerate}


In the first category, Rajan and Davidson~\cite{rajan89corner} produce a number
of elementary test images with a very small number of corners (1 to 4) to test
the performance of detectors as various parameters are varied. The parameters
are corner angle, corner arm length, corner adjacency, corner sharpness,
contrast and additive noise. The positions of detected corners are tabulated
against the actual corner positions as the parameters are varied.  Cooper
\etal~\cite{cooper91corner,cooper-corner} use a synthetic test image consisting
of regions of uniform intensity arranges to create L-, T-, Y-  and X-shaped
corners. The pattern is repeated several times with decreasing contrast.
Finally, the image is blurred and Gaussian noise is added.  Chen
\etal~\cite{chen97corner} use a related method. A known test pattern is
subjected to a number random affine warps and contrast changes. They note that
this is na\"\i{}ve, but tractable.  They also provide an equivalent to the ROC
(Receiver Operating Characteristic) curve.  Zhang \etal~\cite{zhang94corner2}
generate random corners according to their model and plot localization error,
false positive rate and false negative rate against the detector and generated
corner parameters.  Luo \etal~\cite{luo98corner} use an image of a carefully
constructed scene and plot the proportion of true positives as the scale is
varied and noise is added for various corner angles.

Mohanna and Mokhtarian~\cite{mohanna-performance} evaluate
performance using several criteria. Firstly, they define a {\it consistent}
detector as one where the number of detected corners does not vary with various
transforms such as addition of noise and affine warping. This is measured by the
`consistency of corner numbers' (CCN):
\begin{equation}
CCN = 100 \times 1.1^{-|n_t - n_o|},
\end{equation}
where $n_t$ is the number of features in the transformed image and $n_o$ is the
number of features in the original image.  This test does not determine the
quality of the detected corners in any way, so they also propose measuring the
accuracy (ACU) as:
\begin{equation}
ACU = 100 \times \frac{\frac{n_a}{n_o} + \frac{n_a}{n_g}}{2},
\end{equation}
where $n_o$ is the number of detected corners, $n_g$ is the number of ground
truth corners and $n_a$ is the number of detected corners which are close to
ground truth corners. Since real images are used, there is no good definition of
ground truth, so a number of human test subjects (\eg 10) familiar with corner
detection in general, but not the methods under test, label corners in the test
images. Corners which 70\% of the test subjects agree on are kept as ground
truth corners.  This method unfortunately relies on subjective decisions.

%Kienzle \etal~\cite{kienzle05interest} use subconscious human perception to
%define corners, and measure the performance of their detector using the area
%under the ROC (receiver operating characteristic) curve.

Remarkably, of the systems above, only
\cite{chen97corner}, \cite{rajan89corner} and \cite{kienzle05interest}
provide ROC curves (or equivalent): otherwise only a single point (without
consistency on either axis of the ROC graph) is measured.

In the second category, Trajkovic and Hedley~\cite{Trajkovic-Headley-fast}
define stability as the number of `strong' matches (matches detected over
three frames in their tracking algorithm) divided by the total number of
corners.  Tissainayagama and Suterb~\cite{assess-peformance-corner} use a
similar method: a corner in frame $n$ is stable if it has been successfully
tracked from frame 1 to frame $n$. Bae \etal~\cite{bae2002cop} detect optical
flow using cross correlation to match corners between frames and compare the
number of matched corners in each frame to the number of corners in the first
frame.  

To generalize the system performance, the performance can be computed using a
part of a system. For instance, Mikolajczyk and Schmid
\cite{schmid-2005-performance} test a large number of interest point descriptors
and a small number of closely related detectors by computing how accurately
interest point matching can be performed. Moreels and
Perona~\cite{moreels07evaluation} perform detection and matching experiments
across a variety of scene types under a variety of lighting conditions. Their
results illustrate the difficulties in generalizing from system performance
since the best detector for a given descriptor varies with both the descriptor
and lighting conditions.



In the third category, Schmid \etal~\cite{schmid2000comparing} propose that when
measuring reliability, the important factor is whether the same real-world
features are detected from multiple views.  For an image pair, a feature is
`detected' if it is extracted in one image and appears in the second. It is
`repeated' if it is also detected nearby in the second. The repeatability is the
ratio of repeated features to detected features.  They perform the tests on
images of planar scenes so that the relationship between point positions is a
homography.  Fiducial markers are projected onto the planar scene using an
overhead projector to allow accurate computation of the homography.
To measure the suitability of interest points for further processing, the
information content of descriptors of patches surrounding detected points is
also computed. 






